Reframing LLM Agent Security as an Agent-Human Interaction Problem

We argue that LLM agent security is fundamentally an agent-human interaction (AHI) problem, not a purely algorithmic one. To substantiate this position, we conduct a systematic analysis of 59 academic papers, 21 production agent systems, and 26 security plugins as of April 2026. Our analysis reveals a striking pattern: the three widely deployed human-centric security mechanisms (policy specification, runtime approval, and scope configuration) dominate industry practice, each adopted by at least 14 of 21 systems (14, 15, and 16, respectively), while the categories most heavily studied in academia (intent anchoring and trust labeling) see zero production deployment. Yet current human participation mechanisms are far from satisfactory: they suffer from a fundamental trade-off between cognitive burden and security guarantees, leaving users caught between approval fatigue and uncontrolled agent autonomy. We make three contributions. First, through a systematic comparison of LLM-based and human-based intent alignment, we argue that human participation in agent security decisions is indispensable given current capabilities. Second, we quantify a pronounced industry-academia mismatch: the security mechanisms that practitioners actually deploy receive scant research attention, while the approaches that researchers favor remain undeployed. Third, we propose a three-direction research agenda and call for AHI security to be recognized as a first-class research citizen, one that demands its own design principles, evaluation methods, and theoretical foundations.

==> sections/2-0-sok-intro.tex <==
\section{Systematization of \ahisec}
\label{sec:sok}

Defending an LLM agent against a malicious prompt is not a purely algorithmic
problem. Every production agent we examined---from CLI coding assistants to
enterprise orchestration platforms---keeps a human somewhere in the security
loop: the user who clicks \emph{approve}, the developer who writes
\texttt{CLAUDE.md}, the administrator who defines a sandbox profile, or simply
the prompt author whose task description implicitly bounds what the agent is
allowed to do. We collectively call these mechanisms \emph{agent--human
interaction security} (\ahisec).

Despite \ahi{} being the \emph{de facto} defense of deployed agents, the
literature has not systematized it. Existing surveys organize attacks and
defenses along adversarial axes (prompt-injection taxonomies, IFC models,
tool-use threats), leaving the role of the human implicit. We address this gap
by analyzing \npapers academic papers, \nsystems production agent systems, and
\nplugins security plugins collected through \datayear, and distilling five
categories of \ahi{}:

\begin{itemize}[noitemsep, topsep=1pt, leftmargin=*]
  \item \iconPolicySpec~\textbf{Policy Specification}---humans author rules that
  constrain agent behavior (NL policies, DSLs, permission manifests).
  \item \iconTrustLabel~\textbf{Trust and Data Labeling}---humans (or proxies) assign
  trust labels to data sources, propagated through agent execution.
  \item \iconRuntimeApproval~\textbf{Runtime Approval}---humans approve or reject
  specific operations at execution time.
  \item \iconScopeCfg~\textbf{Scope and Boundary Configuration}---humans configure sandboxes,
  resource limits, and access boundaries before execution.
  \item \iconIntentAnchor~\textbf{Intent Anchoring}---the user's task description
  itself is treated as an implicit security anchor for runtime checks.
\end{itemize}

The remainder of this
section first describes our systematization methodology
(\S\ref{sec:sok-methodology}), then walks through each category in
\textbf{order of industry adoption}---from the most widely deployed
(runtime approval, 15/\nsystems systems) to the two zero-adoption categories
(trust labeling and intent anchoring)---to foreground the
academia--industry gap that motivates our empirical study.



==> sections/2-1-methodology.tex <==
\subsection{Systematization Methodology}
\label{sec:sok-methodology}

\noindent\textbf{Scope.} We define \ahi{} as any mechanism in which a human
explicitly or implicitly participates in a security-relevant decision made by,
or about, an LLM agent. This includes pre-deployment decisions (writing a
policy, configuring a sandbox), runtime decisions (approving a command,
labeling a data source), and implicit decisions (expressing intent through a
task prompt). We exclude purely automated defenses with no human in the loop
(e.g., attack classifiers without human review) and pure attack papers without
a corresponding defense contribution.

\noindent\textbf{Data sources.} We drew from three sources to capture both the
state of the art and the state of practice. (i) \emph{Academic papers}: we
searched the 2022--\datayear proceedings of top-tier security (USENIX~Sec,
S\&P, CCS, NDSS), systems (OSDI, SOSP, ASPLOS), ML (NeurIPS, ICML, ICLR),
software-engineering (ICSE, FSE), and NLP (ACL, EMNLP) venues, as well as
arXiv, using keywords drawn from an initial seed set of \ahi{}-relevant papers.
This yielded \npapers papers. (ii) \emph{Production agent systems}: we
catalogued \nsystems widely used coding, computer-use, and enterprise agent
platforms, drawing security-relevant details from official documentation,
engineering blogs, system cards, and public incident reports. (iii)
\emph{Security plugins and tools}: we collected \nplugins open-source and
commercial tools explicitly marketed for agent security, including MCP
scanners, guardrail frameworks, and governance toolkits.

\noindent\textbf{Coding procedure.} Two researchers independently performed
open coding on a random 20\% sample of papers and systems, then met to reconcile
codes into an axial-coding schema. The resulting five categories emerged as the
minimal covering set that accounted for every observed \ahi{} mechanism; each
category was then refined with orthogonal analysis dimensions (e.g., granularity,
enforcement reliability, temporality). The remaining 80\% of the corpus was
coded by one researcher with spot-checks from the second. Disagreements were
resolved through discussion. Most systems and papers exhibit multiple
categories; we record all applicable categories rather than forcing a single
label.

\noindent\textbf{Presentation order.} Following the \emph{adoption-descending}
convention announced in \S\ref{sec:sok}, subsequent subsections cover
runtime approval (\S\ref{sec:sok-c3}), scope configuration (\S\ref{sec:sok-c4}),
policy specification (\S\ref{sec:sok-c1}), trust labeling (\S\ref{sec:sok-c2}), and
intent anchoring (\S\ref{sec:sok-c5}), before a cross-category synthesis
(\S\ref{sec:sok-cross}).


==> sections/2-2-c3-approval.tex <==
\subsection{\iconRuntimeApproval~Runtime Approval}
\label{sec:sok-c3}

\noindent\textbf{Definition.} Runtime approval encompasses mechanisms that pause
agent execution at runtime and defer the decision to allow, reject, or modify
an action to a human. Every major production agent we examined
(15/\nsystems) ships at least one runtime approval mechanism, making it the
default way deployed systems keep humans in the security loop.

\noindent\textbf{Analysis dimensions.} We characterize runtime approval
mechanisms along six orthogonal dimensions summarized in
Table~\ref{tab:c3-dims}: the \emph{object} being approved (individual command,
tool call, plan, or file diff), the \emph{granularity} of the approval
request, the \emph{trigger condition} (always, risk-adaptive, blocklist
match), the \emph{options} offered to the user (binary, three-way with edit,
tiered), the \emph{fatigue-mitigation} mechanism, and how much
\emph{information} about the action is presented to the user at decision
time.

\input{sections/tables/c3-dimensions}

\noindent\textbf{Landscape.} Five academic
papers~\cite{wu2024isolategpt,li2025ace,zhong2025rtbas,shan2026don,wu2025towards}
contribute principled designs for runtime approval: IsolateGPT batches
cross-app interactions for a single decision, ACE asks the user to validate
an \emph{abstract plan} rather than individual calls, RTBAS learns to skip
low-risk approvals (preventing all targeted attacks with only 2\% utility
loss), OpenClaw HITL adds human checkpoints on risky operations, and
AutoPermissions~\cite{wu2025towards} predicts user approval decisions
with 85.1\% accuracy from context. Production systems converge on a narrow
design space: per-command binary prompts with an ``always allow'' memory
(\claudecode, Cursor, Manus, Copilot CLI), occasionally paired with a
sandbox-based auto-approval fast path that reportedly reduces prompts by 84\%
in \claudecode~\cite{anthropic2025claudecode}. MCP proxies
(mcp-guardian~\cite{mcpguardian2025}, Intercept~\cite{intercept2025}) extend
the same pattern to tool-level granularity.

\noindent\textbf{Deep comparison: information and fatigue.} The three dominant
fatigue-mitigation patterns trade off security and usability very differently.
\emph{``Always allow''} (\claudecode, Manus) shifts the burden to the user
once but permanently expands the trusted surface---a silent instance of
\emph{scope creep} (\S\ref{sec:sok-c4}). \emph{Sandbox auto-approval}
(\claudecode, \codex, Copilot CLI) keeps the surface bounded by delegating
the decision to an \emph{orthogonal} mechanism (scope configuration), but only works
when the sandbox itself is correctly configured. \emph{Risk-adaptive
screening} (RTBAS) is the only approach that claims to preserve both low
burden and high security, but has not been adopted by any production system
we surveyed. Information presentation is equally uneven: ChatGPT shows only
``Allow this action?'', \claudecode{} shows raw commands or diffs, and only a
handful of systems (Gemini CLI, RTBAS, MS Agent Framework) surface \emph{why}
an action is considered risky.

\takeaways{\label{tk:c3-fatigue}%
Runtime approval is the industry default (15/\nsystems) but every deployed
fatigue-mitigation mechanism---``always allow'', sandbox auto-approval, YOLO
mode---either expands the trusted surface silently or requires the user to
correctly configure an orthogonal mechanism. The only principled alternative,
risk-adaptive approval, remains academic. \emph{This motivates RQ2.5--RQ2.7:
how users actually use these fatigue-mitigation options, and whether they
understand the security consequences of choosing one.}
}


==> sections/2-3-c4-scope.tex <==
\subsection{\iconScopeCfg~Scope \& Boundary Configuration}
\label{sec:sok-c4}

\noindent\textbf{Definition.} Scope configuration mechanisms let a human define---before or during execution---the set of tools, files, network hosts,
and runtime environments an agent is allowed to touch. 16/\nsystems production
systems ship at least one scope configuration feature, making it the single most
commonly deployed form of \ahi{} when counted at the category level.

\noindent\textbf{Analysis dimensions.} Table~\ref{tab:c4-dims} summarizes six
dimensions: the \emph{object} being bounded (tools, files, network, execution
environment, repos, APIs), \emph{how} the boundary is defined (CLI flags,
config files, GUI, sandbox mode, OAuth scope), the \emph{granularity}
(global mode, per-resource, per-tool, per-parameter), the
\emph{enforcement level}, the \emph{default stance} (open, partial, closed,
tiered), and the boundary's \emph{mutability} during a session.

\input{sections/tables/c4-dimensions}

\noindent\textbf{Landscape.} Scope configuration is the category where academia and
industry are closest in spirit. Academic proposals such as
IsolateGPT~\cite{wu2024isolategpt}, MiniScope~\cite{zhu2025miniscope},
FaultTolerantSandbox~\cite{yan2025fault}, and
AgentBound~\cite{buhler2025securing} formalize principled isolation (app
separation, least-privilege hierarchies, transactional file systems,
permission manifests). Production systems operationalize these ideas at
very different enforcement levels: application-level blocklists in
\claudecode{}, OS-level sandboxing via macOS Seatbelt and Linux Bubblewrap
(\claudecode, \codex{}, Gemini CLI~\cite{google2025geminicli}), VM-level
isolation (Manus, Devin~\cite{devin2025cognition}, Google
ADK~\cite{google2025adk} gVisor), and cloud-platform IAM (Amazon Bedrock
Agents~\cite{aws2025bedrock}).

\noindent\textbf{Deep comparison: default stance and scope creep.} Default
stance sharply separates the design space. \emph{Default-closed} systems
(\codex{}, Gemini CLI, Copilot CLI~\cite{github2025copilotcli}) prioritize
safety but force users to configure the sandbox before real work. \emph{Default-open} systems (\aider~\cite{aider2025}; Replit Agent's early
YOLO mode~\cite{replit2025agent}) are frictionless but have produced real
incidents, including Replit's July 2025 production-database deletion.
\emph{Default-partial} systems (\claudecode, Cursor~\cite{cursor2025security})
sit in between. Across all three stances we observe a subtler problem:
\emph{scope creep}. Every runtime approval ``always allow'' click, every
``permission expansion dialog'' acknowledgement, and every session-wide
Copilot CLI authorization monotonically widens the trusted surface with no
principled shrink-back. Only Cursor Admin and OpenClaw expose bidirectional
policy adjustment; most systems are \emph{expand-only} at runtime.

\takeaways{\label{tk:c4-scope}%
Scope configuration is deployed at every enforcement layer from application to cloud
platform, yet nearly every production system we studied is
\emph{expand-only}: ``always allow'' and session-wide authorizations silently
enlarge the trusted surface with no way to shrink it back. Default stance
further bifurcates the design space into safe-but-frictional and
frictionless-but-incident-prone camps. \emph{This motivates RQ2.8--RQ2.9:
whether users notice their sandbox boundaries drifting, and how they reason
about the relationship between sandbox choice and actual risk.}
}


==> sections/2-4-c1-policy.tex <==
\subsection{\iconPolicySpec~Policy Specification}
\label{sec:sok-c1}

\noindent\textbf{Definition.} Policy specification mechanisms let a human write rules
that constrain agent behavior---who may author them, what they constrain, and
how they are enforced. It is the most \emph{formally studied} \ahi{}
category (13 academic papers) and one of the most widely deployed (14/\nsystems
systems), but academia and industry have diverged sharply in how policies
are expressed and enforced.

\noindent\textbf{Analysis dimensions.} We identify five dimensions
(Table~\ref{tab:c1-dims}): the \emph{author} (end user writing natural-language
rules, developer writing DSL or config, security expert authoring
ABAC/MAC rules, or an LLM generating policy subject to human review), the
\emph{granularity} (coarse global constraints, per-tool, per-parameter,
context-dependent), the \emph{enforcement mechanism}, the \emph{representation}
(natural language, declarative config, DSL, code, permission manifest), and
the \emph{temporality} (static, session-scoped, dynamically evolving).

\input{sections/tables/c1-dimensions}

\noindent\textbf{Enforcement reliability is the primary axis.} We classify
enforcement along a reliability spectrum: \emph{LLM self-compliance} (policy
is a prompt fragment; reliable iff the model chooses to obey), \emph{LLM-as-checker} (a second model policies the first), \emph{deterministic engine}
(independent runtime interpreter, not derivable from model weights),
\emph{framework hook} (in-process callback), and \emph{OS/system} (kernel- or
container-level). Academic proposals dominate the high-reliability end:
Progent~\cite{shi2025progent} and AgentSpec~\cite{wang2026agentspec} interpret
DSL policies deterministically; NeMo Guardrails~\cite{rebedea2023nemo} uses
Colang; CSAgent~\cite{gong2025csagent} and AgentBound~\cite{buhler2025securing}
formalize permission models; SEAgent~\cite{ji2026taming} and
SAGA~\cite{syros2026saga} add MAC/ABAC-style enforcement. Production systems
sit overwhelmingly at the low-reliability end: \claudecode{}'s
\texttt{CLAUDE.md}, \cursorsys's \texttt{.cursorrules}, and \devin's planning
instructions are all natural-language prompt fragments whose enforcement is
self-compliance by the underlying LLM.

\noindent\textbf{Deep comparison: \texttt{CLAUDE.md} vs. Progent vs. Hooks.}
Three representative designs span the space. \texttt{CLAUDE.md} is
zero-friction to author (any end user can write a paragraph) but offers no
guarantees---a prompt injection that contradicts it can win. Progent's DSL
is author-friendly only for developers but compiles to a deterministic
runtime check that cannot be bypassed by prompt injection. \claudecode{}
Hooks sit in the middle: a user writes JavaScript/Python callbacks that
the framework invokes on every tool call, giving deterministic enforcement
but requiring code-level expertise. The existence of all three patterns
\emph{simultaneously} on the same platform suggests developers are
unwilling to choose, forcing end users to absorb the unreliability of
self-compliance by default.

\takeaways{\label{tk:c1-policy}%
Academia overwhelmingly proposes deterministic DSL/formal policy engines,
while 14/\nsystems production systems expose natural-language policy whose
enforcement reduces to LLM self-compliance. The tradeoff is framed as
authorability vs. reliability, but in practice end users inherit the less
reliable default without being told so. \emph{This motivates RQ1.3--RQ1.4
(why developers choose NL over formal policy) and RQ2.3 (whether users
understand that \texttt{CLAUDE.md}-style policies are advisory rather than
enforceable).}
}


==> sections/2-5-c2-labeling.tex <==
\subsection{\iconTrustLabel~Trust \& Data Labeling}
\label{sec:sok-c2}

\noindent\textbf{Definition.} Trust labeling mechanisms let a human (or a
human-configured proxy) annotate data sources with a \emph{trust} or
\emph{integrity} label, then propagate that label through agent execution so
that downstream actions can be gated on the label. This is the category
where academia and industry have diverged most dramatically: we identified
8 academic papers proposing trust labeling designs, but
\textbf{\emph{zero}} of the \nsystems production systems we surveyed adopt
trust labeling as a user-facing security mechanism.

\noindent\textbf{Analysis dimensions.} Table~\ref{tab:c2-dims} lists six
dimensions: \emph{what} is labeled (data, tools, agents, flows), the
\emph{type} of label (binary trusted/untrusted, lattice, capability, or
structured like $\langle\text{cap},\text{conf},\text{trust}\rangle$),
\emph{propagation} rules (deterministic taint, selective, learned), the
\emph{subject} who assigns labels, the \emph{enforcement}, and
\emph{completeness} (full manual, partial+default-deny, incremental).

\input{sections/tables/c2-dimensions}

\noindent\textbf{Landscape.} Academic proposals span the reliability
spectrum. Fides~\cite{costa2025securing} and SafeFlow~\cite{li2025safeflow}
build full information-flow control for agents; CaMeL~\cite{debenedetti2025defeating}
and PFI~\cite{kim2025prompt} enforce prompt-flow integrity by quarantining
untrusted content; AgentArmor~\cite{wang2025agentarmor} performs program
analysis over agent traces; PermissiveIFC~\cite{siddiqui2024permissive}
and f-secure-IFC~\cite{wu2024system} deliberately relax the labeling
burden; VerifiablySafe~\cite{doshi2026towards} adds formal
verification. By contrast, \emph{no production system} ships a user-facing
trust-labeling workflow. The closest analogues are (i) MCP scanners
(\texttt{mcp-scan}~\cite{mcpscan2025}) that \emph{generate} risk reports
users then consult, and (ii) internal architecture-level labels the user
never sees (e.g., Einstein Trust Layer in
Salesforce~\cite{salesforce2025agentforce}).

\noindent\textbf{Deep comparison: labeling burden is not the whole story.}
One natural hypothesis is that full IFC is too costly for end users;
PermissiveIFC and CaMeL were designed specifically to lower the burden
(incremental labeling, default-deny with selective propagation). Yet even
the low-burden variants have zero industry uptake, suggesting the barrier is
not just cost but \emph{mental model}: users do not intuitively reason
about data sources as carriers of trust. In contrast, runtime approval---which
asks users to make a \emph{per-action} judgment---is universally adopted
despite causing approval fatigue. The asymmetry is telling: approving one
command is more concrete than labeling one data source, even if the
cumulative workload of approvals is much larger.

\takeaways{\label{tk:c2-gap}%
8 academic papers, \emph{zero} production systems: trust labeling is the
most dramatic academia--industry gap we observed. Low-burden variants
(CaMeL, PermissiveIFC) have not been adopted either, suggesting the
obstacle is users' \emph{mental model of trust}, not just labeling effort.
\emph{This motivates RQ1.5 (how developers of production systems view
trust labeling) and RQ2.4 (whether users can reason about trust at the
level of data sources rather than individual actions).}
}


==> sections/2-6-c5-intent.tex <==
\subsection{\iconIntentAnchor~Intent Anchoring (Implicit \ahi{})}
\label{sec:sok-c5}

\noindent\textbf{Definition.} Intent anchoring is the only \emph{implicit} \ahi{}
category: rather than asking the user to perform a security action, the
system treats the user's normal task description---the prompt itself---as a
security anchor, and flags runtime behavior that deviates from it. As with
trust labeling, academia has proposed several intent anchoring designs
(5 papers), while \textbf{zero} production systems adopt the idea.

\noindent\textbf{Analysis dimensions.} We characterize intent anchoring along
four dimensions (Table~\ref{tab:c5-dims}): the \emph{anchor source}
(a single user prompt, a query plus dynamically derived rules, or a history
of legitimate behavior), the \emph{deviation-detection} method (semantic
alignment check, program analysis, provable guarantee, rule-based), the
enforcement point, and the \emph{user awareness} level.

\input{sections/tables/c5-dimensions}

\noindent\textbf{Landscape.} TaskShield~\cite{jia2025task} and
MELON~\cite{zhu2025melon} take the user prompt as a ground-truth task
specification and score every agent action against it, blocking those
that cannot be justified by the declared task. DRIFT~\cite{li2025drift}
compiles dynamic security rules from the query and monitors execution.
AGrail~\cite{luo2025agrail} learns lifelong safety checks.
Agent-Sentry~\cite{sequeira2026agent} treats the original user request as
trusted input and audits provenance.
AgentGuardian~\cite{abaev2026agentguardian} learns normal behavior from a
staging phase and treats deviations as suspicious. None of these designs
require the user to configure anything or click any prompt---security
enforcement is invisible.

\noindent\textbf{Why is invisible security not adopted?} Our reading of
production documentation offers two plausible hypotheses. First, the
same property that makes intent anchoring user-friendly---invisibility---makes
it difficult to \emph{market}, since users do not perceive a new safeguard.
Second, task intent is notoriously ambiguous, and a false-positive block
(agent refuses a legitimate follow-up) is hard to explain to a user who
never asked for a security check in the first place. Neither hypothesis
has been empirically tested.

\takeaways{\label{tk:c5-intent}%
Intent anchoring is the second zero-adoption category: 5 papers, 0/\nsystems
systems. Unlike trust labeling, its user burden is \emph{already zero}, so
cost cannot be the explanation. We hypothesize that invisibility and
false-positive attribution are the blockers. \emph{This motivates RQ1.11
(whether developers consider user prompts a credible anchor) and RQ2.10
(whether users would want to know their prompt is being used for security
purposes).}
}


==> sections/2-7-cross-category.tex <==
\subsection{Cross-Category Analysis}
\label{sec:sok-cross}

\input{sections/tables/cross-category}

Having walked through Policy Specification--Intent Anchoring individually, we now step
back and ask three comparative questions: \emph{how widely is each category
adopted?}, \emph{how do they combine in practice?}, and \emph{what does the
overall picture imply for users?}

\noindent\textbf{Adoption gap.} The bifurcation is
stark: runtime approval and scope configuration are near-universal in production
(15/\nsystems and 16/\nsystems respectively) while attracting modest
academic attention; policy specification is heavily studied in academia \emph{and}
adopted by industry, but with \emph{different} representations (deterministic
DSLs in papers vs.\ natural-language prompts in systems); trust labeling and
intent anchoring together account for 13 academic papers but \emph{zero}
industry adoption. Table~\ref{tab:cross-cat} reports the exact counts and
lists, for each cell, the enforcement layers where the category is
instantiated.


\noindent\textbf{How categories combine.} Production systems do not pick a
single category; they stack three or four, with runtime approval+scope configuration+policy specification being the dominant combination (\claudecode, \codex,
Cursor, Gemini CLI, Copilot CLI all follow this pattern).
Runtime approval+scope configuration form a \emph{complementary pair}: fatigue is
managed by widening the sandbox (reducing how often approval is
needed), while sandbox misconfiguration is backstopped by runtime
approval prompts. Neither mechanism works well in isolation, but stacking
them inherits the weaknesses of \emph{both}: silent scope creep from
runtime approval and expand-only drift from scope configuration.

\noindent\textbf{Security--usability frontier.} Projecting the \nsystems
systems onto a (security, usability) plane reveals three clusters:
(1)~\emph{high-security, high-burden} systems that default closed and ask
frequently (\codex, Gemini CLI, Bedrock Agents~\cite{aws2025bedrock});
(2)~\emph{low-security, low-burden} systems that default open
(\aider, early Replit Agent); (3)~a \emph{middle band} relying on
runtime approval+``always allow'' tradeoffs (\claudecode, \cursorsys,
Copilot CLI). The fourth quadrant---high security \emph{and} low burden---is
occupied only by academic proposals (RTBAS, TaskShield, CaMeL), precisely
the ones industry has not adopted.

\takeaways{\label{tk:cross-gap}%
The academia--industry gap is structured, not uniform. It is largest in
trust labeling and intent anchoring (0 adoption), visible in policy specification
(different representations), and smallest in runtime approval and
scope configuration. The runtime approval+scope configuration combination that industry has
converged on produces the middle-band security--usability profile, while
the methods that could in principle occupy the high-security,
low-burden quadrant remain academic.
}

\takeaways{\label{tk:cross-transition}%
The SoK explains \emph{what} mechanisms exist and \emph{where} the gap lies,
but it cannot answer two empirical questions the gap raises: (i)~why
developers of deployed systems choose the low-reliability-but-familiar
defaults, and (ii)~whether users can actually operate the mechanisms they
inherit. These questions motivate the research agenda proposed in the remainder of
this paper.
}


==> sections/3-study-design.tex <==
\section{Study Design}
\label{sec:study-design}

\peiran{Study design placeholder. To be written after Related Work.}


==> sections/4-results.tex <==
\section{Results}
\label{sec:results}

\peiran{Results placeholder. Empirical data to be added after interview and survey collection.}


==> sections/5-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\peiran{Discussion placeholder. Key findings, design implications, limitations.}


==> sections/6-related-work.tex <==
\section{Related Work}
\label{sec:related-work}

\peiran{Related Work placeholder. To be written after SoK.}


==> sections/7-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\peiran{Conclusion placeholder.}

